Level-set topology optimization considering nonlinear thermoelasticity

At elevated temperature environments, elastic structures experience a change of the stress-free state of the body that can strongly influence the optimal topology of the structure. This work presents level-set based topology optimization of structures undergoing large deformations due to thermal and mechanical loads. The nonlinear analysis model is constructed by multiplicatively decomposing thermal and mechanical effects and introducing an intermediate stress-free state between the undeformed and deformed coordinates. By incorporating the thermoelastic nonlinearity into the level-set topology optimization scheme, wider design spaces can be explored with the consideration of both mechanical and thermal loads. Four numerical examples are presented that demonstrate how temperature changes affect the optimal design of large-deforming structures. In particular, we show how optimization can manipulate the material layout in order to create a counteracting effect between thermal and mechanical loads, even up to a degree that buckling and snap-through are suppressed. Hence the consideration of large deformations in conjunction with thermoelasticity opens many new possibilities for controlling and manipulating the thermo-mechanical response via topology optimization.

==> includes/Intro.tex <==
\section{Introduction}

Thermoelasticity broadly refers to a coupled phenomenon where the elastic responses of a structure are affected by a temperature change. 
The phenomenon is widely considered in diverse engineering disciplines in association with various structural responses, ranging from elastic behaviors such as classical volumetric expansion to the deterioration of the structural integrity such as thermal buckling, delamination, and fracture. 
Recently, thermoelastic behaviors have also been employed to realize non-conventional behavior of materials, e.g., metamaterials \cite{qu2017micro, wu2016isotropic}, and phase-changing smart materials \cite{yuan2017shape, de2014programmed}. 

Topology optimization of structures experiencing thermoelastic load was first studied by Rodrigues and Fernandes \cite{Rodrigues1995}, where the classical compliance objective was extended to accomodate thermal load combined with mechanical loads. 
Therein, a design scheme that follows the material distribution approach with homogenization was presented.
Such a coupled load was later considered also with other approaches, such as Evolutionary Structural Optimization, or ESO \cite{Li2001}; and the level-set method \cite{Xia2008}.
By solving the thermo-compliance minimization problem, these schemes demonstrated how optimized structures accommodate a uniform temperature change. 
Due to its simplicity and analogy with the classical structural compliance minimization problem, thermo-compliance minimization has been widely adopted in later works, including design that involves multi-material \cite{Gao2016} and coupled physics \cite{de2007topological}. 

To further discuss structural resistance to thermoelastic loads, Pedersen and Pedersen \cite{Pedersen2010} presented topology optimization considering mechanical strength, where they identified that different ratios between mechanical and thermal loads lead to different designs.   
In the same line of thought, Deaton and Grandhi \cite{Deaton2013} examined the difference between optimized layouts that are derived based on the different definitions of the compliance. 
Therein thermal and mechanical compliances are defined as $\boldsymbol{u}^{thT} \boldsymbol{f}^{th}$, and $\boldsymbol{u}^{mT} \boldsymbol{f}^m$, where $\boldsymbol{u}$ and $\boldsymbol{f}$ represent the nodal displacement and the load vector, respectively. 
Superscripts $th$ and $m$ indicate that the terms are either thermal or mechanical. 
Comparative studies were also conducted by Zhang et al., \cite{Zhang2014}, where the topological layouts resulting either from strain energy minimization or mean compliance minimization are compared and discussed. 
These lead to a search of alternative thermoelastic merit functions, such as a constraint on local stress concentration \cite{Takalloozadeh2017, Neiferd2018}, and a thermoelastic buckling constraint \cite{deng2017topology}.

\color{black}
Multifunctional actuators and metamaterials, 
that are designed to exhibit a thermally driven shape change by 
% which designs thermally-driven shape change 
by meticulously distributing active materials, are another class of applications of topology optimization considering thermoelasticity. 
\color{black}
In the seminal works by Sigmund and Torquato \cite{sigmund1997design}, and Sigmund \cite{sigmund2001designI, sigmund2001designII}, metamaterials of negative thermal expansion, and micro-electromechanical actuators are designed, respectively. 
The idea of thermally driven actuation and multiphysical coupling has been widely explored thereafter, leading to the works including the extensions to different topology optimization approaches \cite{luo2009shape, luo2012meshfree}, the designs of piezo-electric actuators \cite{ruiz2018optimal, ruiz2018optimal_math, kogl2005topology, carbonari2005design}, and the designs of recent 4D printed structures that exhibit self-morphing behavior \cite{maute2015level, geiss2019combined}.

Structures may experience thermoelastic loads that induce a large deflection of the structure, e.g., kinetic heating in aerostructures \cite{Deaton2015}. 
In such cases, nonlinear thermoelasticity must be considered, meaning that the infinitesimal strain should be replaced with nonlinear strain; 
otherwise, displacement and stress states obtained by structural analysis are highly overestimated due to the neglected stress-stiffening effect, and these inaccurate variables potentially lead to non-optimal structures \cite{chung2019nonlinear}. 
Such an inaccuracy is exacerbated when temperature change is involved \cite{Deaton2015, chung2015light} as the thermoelastic behavior incorporates the temperature-induced deformation that in effect changes the stress-free state with respect to the undeformed state \cite{Lubarda2004}. 

\color{black}
In the topology optimization perspective, the major issues and challenges concerning the incorporation of the nonlinear analysis model to the optimization scheme have been identified in the pioneering works \cite{sigmund2001designI, sigmund2001designII, ruiz2018optimal}.
Thermally-driven compliant mechanisms are designed by introducing nonlinear thermoelasticity in these works. 
A coupled problem where nonlinear elasticity and thermal modeling are combined has been incorporated into the optimal layout design in a single-material \cite{sigmund2001designI} and multimaterial configuration \cite{sigmund2001designII}. 
These works have been recently extended to the piezoelectric gripper considering out-of-plane deformation \cite{ruiz2018optimal}.
Therein, the effect of the nonlinearity has been demonstrated by comparing the shapes and the optimalities of these designs with the corresponding linear solutions. 
% In these early works, it is shown that the incorporated nonlinearity does influence the material distribution, but they do not discuss large deformation induced by mechanical loading, with the co-presence of temperature change.  
However, when a mechanical load also potentially induces a large deformation in the thermoelastic design problem, the investigation of the combined load becomes complex because the effect of the fixed mechanical load is on the contrary to that of thermal load. 
Decreasing volume of the material during the optimization, for example, increases the effect of the mechanical load whereas decreases the amount of the thermal load \cite{Zhang2014}; therefore the optimized material layouts are expected to consider such contradicting effect of combined loads. 
In this work, we present a level-set based topology optimization framework that is able to design thermoelastic structures undergoing large mechanical and temperature loads, while attaining crisp solid-void topologies.
% The presented framework is largely indebted to the early works such as \cite{sigmund2001designI, sigmund2001designII, jog1996distributed}. 
\color{black}

In this respect, the present work is also largely indebted to early works on the optimization 
with nonlinear elasticity under mechanical loading only, which was first considered by Buhl et al. \cite{Buhl2000}. 
The resulting material layouts are shown to deviate from the linear solution as the external load increases. 
A difference between the compliance and complementary work objectives is also evident and the corresponding layout changes are discussed.  
Jung and Gea \cite{Jung2004} further discussed the layout change by examining the separate influence of material and geometric nonlinearities on the optimum layouts.
A recent work by Li et al., \cite{li2018shape} further expands the usage of nonlinear elasticity in topology optimization to design that preserves local geometric features constraining warpage.
Allaire \cite{Allaire2004} and Kwak and Cho \cite{Kwak2005} extended nonlinear topology optimization by using a level-set method. 
Recently, optimum layouts obtained by the nonlinear elastic level-set topology optimization were discussed also in terms of attenuation of local buckling \cite{Chen2017}.

Numerous works were dedicated to topological design of structures devoid of structural instabilities.
Bruns et al. \cite{Bruns2002} proposed a combination of the arc-length scheme with the classical Newton-Raphson solver, in order to robustly converge to a structure that undergoes snap-through. 
Kemmler \cite{Kemmler2005} identified the snap-through phenomenon and loss of stability of the intermediate layouts found during the optimization.
These understandings are later applied to optimizing buckling stiffness \cite{lindgaard2013compliance, Jansen2014}, and designing snapping mechanisms \cite{james2016layout}.
Recently, Wallin et al. \cite{wallin2018stiffness} addressed the structural stability of the optimum layouts depending on the choice of objective function that in effect optimizes different types of stiffness. 

In this work, we formulate and develop nonlinear thermoelastic level-set topology optimization.
In particular, we investigate the intertwined effects of the nonlinearity and thermal loads on optimized structural designs. 
Both geometric and material nonlinearities are considered in the analysis and sensitivity calculation. 
A thermally induced change of the natural state, which significantly affects the stress state, is identified by the multiplicative decomposition of the strain tensor \cite{belytschko2013nonlinear, Lubarda2004, geiss2019combined}.
These nonlinear thermoelastic considerations enhance the accuracy in estimating internal states for higher loading conditions, hence extend the range of both mechanical and thermal loads to the extent where the structure deforms by the same order as its own characteristic dimension. 
The temperature range, for example, roughly coincides with what aero-structures experience under high-temperature operating conditions \cite{Deaton2015}. 
To demonstrate such nonlinear effects, bending-dominant and buckling-dominant structures are examined as a basis for discussing how temperature changes affect the optimum designs. % By investigating the widened range of thermoelastic loads, we found that temperature changes have a profound influence in determining the optimized material layouts, especially when large structural deformations are considered. 
% The optimized distribution of material is shown to balance between a layout that sustains the mechanical load, and the one that manipulates the thermally induced deformation. 
% Furthermore, such an effect is found to be more substantial when structures deform to the nonlinear regime, such as snap-through instability, as the optimized structures are shown to attenuate such nonlinear phenomena.  

The remainder of the paper is organized as follows. 
Section 2 describes the thermoelastic formulation and its corresponding finite element analysis model. 
The Total Lagrangian approach is implemented based on the deformation gradient that is multiplicatively decomposed into its mechanical and thermal parts. 
The optimization problem and the corresponding shape sensitivity used in the level-set topology optimization are presented in Section 3. 
In Section 4 we present four demonstrative examples of which material layouts are discussed in detail, and investigate the combined effect of the nonlinearity and the thermal loads. 
Finally, the conclusion is given in Section 5.  
